GPS: Genetic Prompt Search for Efficient Few-shot Learning

Prompt-based techniques have demostrated great potential for improving the few-shot generalization of pretrained language models. However, their performance heavily relies on the manual design of prompts and thus requires a lot of human efforts. In this paper, we introduce Genetic Prompt Search (GPS) to improve few-shot learning with prompts, which utilizes a genetic algorithm to automatically search for high-performing prompts. GPS is gradient-free and requires no update of model parameters but only a small validation set. Experiments on diverse datasets proved the effectiveness of GPS, which outperforms manual prompts by a large margin of 2.6 points. Our method is also better than other parameter-efficient tuning methods such as prompt tuning.

==> EMNLP 2022/exp.tex <==
\section{Experiments}
\label{sec:exp}

In this section, we conduct extensive experiments to study the effectiveness of GPS, and reveal the way to obtain the best prompt for Genetic Prompt Search. We also study several possible impact factors and hyper-parameters in GPS. 

\subsection{Experimental Setups}
To match with the real few-shot scenario, we use a small validation set randomly sampled from each task.
Empirically, for every task, only 32 data samples are needed to build the validation set, and we keep the number of samples for each task the same to make the data balanced. The actual shot number will be 32 divided by the number of classes. For example, we will have 8 shots for each class if there are 4 classes.
Our few-shot setting follows the ``true few-shot'' setting~\cite{perez2021true}. For all the tuning-free methods that do not require a training set, we use the validation set to search for the optimal prompt.
For all the methods that require tuning parameters, we split the validation set into two halves as a training set and a validation set. Therefore all the experiments use the same number of data for fair comparison. We repeat
the experiments of few-shot methods with 3 different data splits and report the average performance across all prompts.
% and ensure the training and validation set contains same number of samples $|D_{train}| = |D_{val}|$ .


\subsection{Datasets}
% We take 10 of the reserved test tasks in T0, 
We use the 10 test tasks of T0, which are not included in the prompted training tasks, to evaluate the performance of our \proposed and other methods.
There are various kinds of NLP tasks in the test set including natural language inference (ANLI R1, ANLI R2, ANLI R3, CB, RTE), coreference resolution (WSC, Winogrande), sentence completion (COPA, HellaSwag) and word sense disambiguation (WiC). We report the average accuracy of different prompts for all the tasks.


\subsection{Baselines}
We compare \proposed under the few-shot learning setting with state-of-the-art methods. Here we categorize the baselines to three groups: the manual prompt baseline, methods with tunable parameters, and methods without tunable parameters. %  and gradient free methods, 

\textbf{Manual prompt baseline}: T0~\cite{sanh2021multitask} is a multitask pretrained encoder-decoder model, which is on the basis of T5 and further pretrained on different types of downstream tasks with diverse manually designed prompts.

\textbf{Methods w. tunable parameters}: 
1) Model Tuning (MT) is the common paradigm to finetune the entire pretrained language model on each task.
2) Prompt Tuning~\cite{webson2021prompt} (PT) is a gradient-guided tuning method, which only trains the extra continuous soft prompts while the pretrained language model is frozen. 
3) Black-Box Tuning~\cite{sun2022black} (BBT) is a gradient-free few-shot tuning method. Rather than searching for discrete text prompts, Black-Box Tuning aims at searching for the best soft prompt embedding in the continuous space.

\textbf{Methods w.o. tunable parameters}: 
1) In-Context Learning~\cite{NEURIPS2020_gpt3} (ICL) is a common method of few-shot learning for large-scale pretrained language models. Demonstrations  composed of labeled samples and manual templates are used to help the model understand the meaning of the test tasks.
2) GRIPS~\cite{prasad2022grips} is a concurrent work which introduced a gradient-free edit-based method for optimal prompt search, but GRIPS mostly focus on simple rule-based editing operations such as add, deletion and swap. 

% \begin{itemize}
%     \item T0~\cite{sanh2021multitask} is a multitask pretrained encoder-decoder model, which is on the basis of T5 and further pretrained on different types of downstream tasks with diverse manually designed prompts.
%     \item In-Context Learning~\cite{NEURIPS2020_gpt3} (ICL) is a common method of few-shot learning for large-scale pretrained language models. Demonstrations composed of labeled samples and manual templates are used to help the model understand the meaning of the test task.
%     \item Model Tuning (MT) is the common paradigm to finetune the entire pretrained language model on each task.
%     \item Prompt Tuning~\cite{webson2021prompt} (PT) is a gradient-guided tuning method, which only trains the extra continuous soft prompts while the pretrained language model is frozen. 
%     \item Black-Box Tuning~\cite{sun2022black} (BBT) is a gradient-free few-shot tuning method. Rather than searching for discrete text prompts, Black-Box Tuning aims at searching for the best soft prompt embedding in the continuous space.
%     \item GRIPS~\cite{prasad2022grips} is a concurrent work which introduced a gradient-free edit-based method for optimal prompt search. But differently GRIPS mostly focus on simple rule-based editing operations such as add, deletion and swap. 
% \end{itemize}

We conduct experiments on English natural language processing tasks of which the manual prompts are introduced in T0~\cite{sanh2021multitask}. 
Note that all the seed prompts we used in our experiments were taken from T0. To make fair comparison, we used the same suite of prompts for other baseline approaches including Model Tuning, Prompt Tuning, Black-Box Tuning and GRIPS.
% However, the gradient tuning methods also utilize the hard prompts designed by T0, This raise the issue that which seed prompts shall we take in the finetuning phase. Here we only choose 3~5 prompts as our final prompts, and report the average. 

% In our experiment, the 
For Prompt Tuning, we use the Adafactor Optimizer and set the learning rate as 0.05. 
For Model Tuning, we use the same Optimizer as Prompt Tuning and set the learning rate as 5e-5. The batch size is set as 4 for both prompt tuning and model tuning. 
For Black-Box Tuning, we take 500 as the intrinsic dimension, 20 as the pop size and the cross entropy loss. We report the best results with 1 and 50 soft prompt tokens.
For In-Context Learning, we randomly select 2 examples from the training set for each task.
For GRIPS, we try to keep all hyper-parameters the same as \citet{prasad2022grips}. The only difference is that the initial prompts are from T0.


\begin{table*}[t]
\small
\centering
\begin{tabular}{cm{0.45in}<{\centering}m{0.45in}<{\centering}m{0.45in}<{\centering}m{0.45in}<{\centering}m{0.45in}<{\centering}m{0.45in}<{\centering}m{0.45in}<{\centering}m{0.45in}<{\centering}}
\toprule
\multirow{2}{*}{Dataset} & \multicolumn{2}{c}{Zero-Shot} & \multicolumn{3}{c}{Few-Shot Parameter Tuning} & \multicolumn{3}{c}{Few-Shot Parameter Frozen} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-6}
\cmidrule(lr){7-9}
& $\text{T0}^\dag$ & T0 $\ddag$ & BBT & PT & MT & ICL & GRIPS & Our GPS \\
\midrule
ANLI R1    & $43.56$ & $43.16$ & $42.97_{0.32}$ & $43.21_{0.15}$ & $\underline{46.73_{3.25}}$ & $37.87_{0.80}$ & $\mathbf{44.41_{0.01}}$ & $44.06_{2.78}$\\
ANLI R2    & $38.68$ & $38.68$ & $38.89_{0.05}$ & $37.36_{1.69}$ & $\underline{39.12_{3.17}}$ & $34.51_{1.53}$ & $\mathbf{39.57_{0.24}}$ & $38.10_{1.68}$\\
ANLI R3    & $41.26$ & $41.87$ & $41.32_{0.05}$ & $40.85_{0.36}$ & $\underline{42.20_{2.11}}$ & $35.98_{2.80}$ & $\mathbf{42.96_{0.42}}$ & $41.51_{2.33}$\\
CB         & $70.12$ & $70.12$ & $72.06_{0.14}$ & $71.31_{2.39}$ & $\underline{83.97_{5.40}}$ & $59.21_{5.65}$ & $76.55_{0.41}$ & $\mathbf{80.12_{1.61}}$\\
RTE        & $80.83$ & $80.97$ & $81.73_{0.49}$ & $\underline{82.47_{0.86}}$ & $79.51_{2.08}$ & $64.86_{10.29}$ & $81.71_{0.12}$ & $\mathbf{84.22_{1.02}}$\\
WSC        & $61.45$ & $61.06$ & $60.74_{0.31}$ & $63.30_{1.82}$ & $\underline{64.65_{1.79}}$ & $61.03_{3.86}$ & $61.47_{1.44}$ & $\mathbf{63.62_{1.68}}$\\
Winogrande & $59.94$ & $59.70$ & $59.46_{0.32}$ & $58.63_{0.70}$ & $\underline{59.76_{1.47}}$ & $53.22_{1.58}$ & $58.11_{0.26}$ & $\mathbf{59.59_{2.06}}$\\
COPA       & $90.02$ & $90.02$ & $90.51_{0.74}$ & $92.33_{0.39}$ & $\underline{92.54_{0.98}}$ & $82.82_{1.39}$ & $91.75_{0.42}$ & $\mathbf{93.50_{0.14}}$\\
HellaSwag  & $33.55$ & $33.52$ & $33.47_{0.20}$ & $37.28_{0.29}$ & $\underline{49.75_{4.98}}$ & $27.35_{2.28}$ & $33.09_{0.20}$ & $\mathbf{38.85_{5.54}}$\\
WiC        & $56.68$ & $56.13$ & $57.09_{0.40}$ & $58.86_{1.22}$ & $\underline{59.04_{1.09}}$ & $50.35_{0.89}$ & $57.03_{0.67}$ & $\mathbf{57.65_{1.18}}$\\
\midrule
Avg        & $57.60$ & $57.52$ & $57.82_{0.03}$ & $58.56_{0.20}$ & $\underline{61.73_{0.09}}$ & $51.28_{1.66}$ & $58.66_{0.35}$ & $\mathbf{60.12_{1.40}}$\\
\bottomrule
\end{tabular}
\caption{Main results (accuracy) on the test benchmark of different methods. Black-Box Tuning (BBT), Prompt Tuning (PT), Model Tuning (MT) tune the continuous prompt embedding or the full model for few-shot learning, while In-Context Learning (ICL), GRIPS~\cite{prasad2022grips} and our GPS do not update any parameter. We repeat the experiments of few-shot methods with 3 different data splits and report the average performance across all prompts. The number of subscript is the standard deviation across different data splits. T0, BBT, PT, MT, and ICL all use  the same manual prompt set, while GRIPS and GPS use their final searched prompt sets, where the number of prompts are the same in different prompts sets. \underline{Underlined} results are the best of few-shot parameter tuning methods and \textbf{bold} results are the best of few-shot parameter frozen methods. \dag: The original results from \citet{sanh2021multitask}. \ddag: The results we reproduced.}
\label{tab:main_results}
\end{table*}
% \begin{table*}[t]
% \small
% \centering
% \begin{tabular}{cm{0.45in}<{\centering}m{0.45in}<{\centering}m{0.45in}<{\centering}m{0.45in}<{\centering}m{0.45in}<{\centering}m{0.45in}<{\centering}m{0.45in}<{\centering}m{0.45in}<{\centering}}
% \toprule
% \multirow{2}{*}{Dataset} & \multicolumn{2}{c}{Zero-Shot} & \multicolumn{3}{c}{Few-Shot Parameter Tuning} & \multicolumn{3}{c}{Few-Shot Parameter Frozen} \\
% \cmidrule(lr){2-3}
% \cmidrule(lr){4-6}
% \cmidrule(lr){7-9}
% & $\text{T0}^\dag$ & T0 $\ddag$ & BBT & PT & MT & ICL & GRIPS & Our GPS \\
% \midrule
% ANLI R1    & 43.56 & 43.16 & 42.60 & 43.04 & \textbf{49.56} & 37.58 & 44.41 & 46.47\\
% ANLI R2    & 38.68 & 38.68 & 38.94 & 38.19 & \textbf{42.53} & 33.05 & 39.32 & 39.91\\
% ANLI R3    & 41.26 & 41.87 & 41.34 & 40.48 & 42.59 & 38.98 & 42.48 & \textbf{43.01}\\
% CB         & 70.12 & 70.12 & 71.90 & 74.05 & 77.98 & 65.24 & 76.07 & \textbf{80.00}\\
% RTE        & 80.83 & 80.97 & 82.01 & 82.92 & 81.30 & 72.42 & 81.59 & \textbf{83.86}\\
% WSC        & 61.45 & 61.06 & 60.38 & 63.56 & \textbf{65.87} & 64.42 & 61.54 & 65.48\\
% Winogrande & 59.94 & 59.70 & 59.24 & 58.00 & 58.92 & 51.45 & 58.40 & \textbf{61.96}\\
% COPA       & 90.02 & 90.02 & 91.13 & 93.02 & 93.17 & 84.07 & 91.41 & \textbf{93.43}\\
% HellaSwag  & 33.55 & 44.95 & 33.38 & 46.90 & 47.23 & 32.25 & 47.90 & \textbf{51.83}\\
% WiC        & 56.68 & 56.13 & 57.37 & 57.98 & \textbf{59.14} & 49.33 & 57.23 & 58.82\\
% \midrule
% Avg        & 57.60 & 58.67 & 57.83 & 59.81 & 61.83 & 52.88 & 60.03 & \textbf{62.48}\\
% \bottomrule
% \end{tabular}
% \caption{Main results of different methods. Black-Box Tuning (BBT), Prompt Tuning (PT), Model Tuning (MT) tune the continuous prompt embedding or the full model for few-shot learning, while In-Context Learning (ICL), GRIPS~\cite{prasad2022grips} and our GPS do not update any parameter. We report the average performance across all prompts. T0, BBT, PT, MT, and ICL all use  the same manual prompt set, while GRIPS and GPS use their final searched prompt sets, where the number of prompts are the same in different prompts sets. \dag: The original results from \citet{sanh2021multitask}. \ddag: The results we reproduced.}
% \label{tab:main_results}
% \end{table*}

\subsection{Implementation Details}
In practice, we assume there is only a few-shot validation set to conduct our experiments, which means, we will not tune any hyper-parameter in the method according to the performance on test set. Specifically, we set K as the number of initial prompts for each. It is a reasonable setup, because if the K is too low, the method may simply drop all prompts of low quality and keep the rest prompts as the final result. In the main experiment, we run the genetic prompt search for 6 steps. To generate diverse candidate prompts at each step, we perform top-p sampling, where the p is set as 0.9. Besides, we filter out all prompts that are the same as the existing prompts or do not have a valid input placeholder, such as "premise" in SuperGLUE CB.


\subsection{Main Results}

% \subsection{Zeroshot Learning without Updating Parameters}
In this section, we compare \proposed with the aforementioned baselines on the 10 unseen tasks.



% BBT performs worse than PT especially on HellaSwag.
% We observed that Black-Box Tuning, is beaten by the manually designed prompts. This may illustrates that black-box tuning is not stable when the validation set is small.
% Other baselines like prompt tuning and model tuning outperforms black-box tuning easily, since they can update parameters according to the training set, as well as avoid over-fitting with the validation set. These methods can raise the performance a little bit comparing to zero-shot learning baseline. However, but the training set limits the methods to obtain better results.

As shown in Table~\ref{tab:main_results}, \proposed outperforms other few-shot learning methods that do not require parameter updating. Compared to GRIPS, another discrete prompt search method, GPS wins 1.4 points on average, and the performance of GRIPS is close to that of PT while worse than MT. This reveals that the way to conduct prompt generation is important to obtaining the optimal prompts, and we also conduct further ablation studies on different prompt generation strategies in Sec~\ref{subsubsec:prompt_generation_strategies}.
% TODO: 同样，On the other hand不用于转折关系
Meanwhile, we find that the result of ICL with T0 is significantly worse than the zero-shot baseline, which differs from the results in previous works using GPT. We suppose this is because the prompts used in T0 at the multitask pretraining stage are quite different from the ICL demonstrations with labeled examples.
Even compared with parameter-efficient tuning methods like black-box tuning and prompt tuning, \proposed also achieves considerably better performance.



\begin{table}[t]
\small
\centering
\begin{tabular}
{cm{0.25in}<{\centering}m{0.25in}<{\centering}m{0.25in}<{\centering}m{0.3in}<{\centering}m{0.3in}<{\centering}}
\toprule
Dataset & T0\dag & BT & Cloze & SC (GPT2) & SC (T5LM) \\
\midrule
ANLI R1    &43.16 & 44.95 & 42.10 & 44.64 & \textbf{46.47}\\
ANLI R2    &38.68 & \textbf{40.13} & 38.95 & 39.14 & 39.91\\
ANLI R3    &41.87 & 42.83 & 42.00 & 42.75 & \textbf{43.01}\\
CB         &70.12 & 79.38 & 73.21 & 79.71 & \textbf{80.00}\\
RTE        &80.97 & 82.60 & 82.64 & 82.53 & \textbf{83.86}\\
WSC        &61.06 & 65.38 & 64.38 & 63.65 & \textbf{65.48}\\
Winogrande &59.70 & 61.09 & 53.50 & 59.76 & \textbf{61.96}\\
COPA       &90.02 & 93.12 & 89.77 & 93.31 & \textbf{93.43}\\
HellaSwag  &33.52 & 36.34 & 33.83 & 36.72 & \textbf{44.29}\\
WiC        &56.13 & \textbf{60.72} & 56.15 & 57.91 & 58.82\\
\midrule
Avg        &57.52 & 60.65 & 57.65 & 60.01 & \textbf{61.72}\\
\bottomrule
\end{tabular}
\caption{Ablation results with different prompt generation strategies including Cloze, Back Translation (BT) and Sentence Continuation (SC). For SC, we include two different pretrained models, GPT2 and T5LM. \dag: The results we reproduced.}
\label{tab:ablation_prompt_generation_strategies}
\end{table}


% \subsection{}
% Secondly, to understand the importance of Prompt Search, we compare the \proposed with several prompt learning approaches that do not require updating parameters, like how will the GPS perform with Prompt-tuning, Model tuning or Blackbox tuning. 

\subsection{Ablation Study}
In this section, we conduct several ablation experiments on various hyper-parameters. To control experimental variables, we explore the effect of each hyper-parameter while keeping the other hyper-parameters fixed as the default value. 
% To stabilize the experimental results and reduce the variance over different runs, each experiment is performed on the same data split with different random seeds for five runs and report the average.   
% We will experiment on the factors and affect the performance of Genetic Prompt Search like models used to generate prompts, the size of our tiny validation set and number of iterations for GPS. 

\subsubsection{Prompt Generation Strategies}
\label{subsubsec:prompt_generation_strategies}

In Table~\ref{tab:ablation_prompt_generation_strategies}, we compare different automatic prompt generation strategies, including Cloze, Back Translation (BT), and Sentence Continuation (SC) as described in section~\ref{subsection:prompt_generation}. Among all the prompt generation strategies, SC with T5LM obtains the best results. And SC with T5LM shows that it outperforms SC with GPT2 by a significant margin. This reveals that the pretrained model for SC is vital to obtaining the optimal prompts, and larger language models usually generate better prompts. 

BT achieves good results and has the best score on ANLI R2 and WiC. Cloze does not work well and its overall performance is no better than the zero-shot baseline. The results suggest that these simple strategies cannot provide enough variance of prompts for search, and we will discuss this with a few examples in section~\ref{sub:case_study}. 

% SC with T5LM shows the best performance among these strategies and outperforming SC with GPT2 by a large margin. It 

% 英文prompt的case
% \begin{table*}[t]
% \small
% \centering
% \begin{tabular}{m{2cm}<{\centering}p{10cm}m{1.5cm}<{\centering}}
% \toprule
% \textbf{Task} & Prompts & Improve. \\
% \midrule
% \multirow{4}{*}{\makecell[c]{\\ Hellaswag}} & \textbf{Origin}: If a description of a situation begins like this: \{\{ ctx \}\}... Then how does it continue? & \multirow{4}{*}{\makecell[c]{\\5.40}} \\
% ~ & \textbf{BT}: - & ~ \\
% ~ & \textbf{GPT2}: - & ~ \\
% ~ & \textbf{T5}:  If the description of a situation begins like this: \{\{ ctx \}\}... then what is it doing? & ~ \\
% \midrule
% \multirow{4}{*}{\makecell[c]{\\SuperGLUE \\ COPA}} & \textbf{Origin}: Select the most plausible \{\% if question == "cause" \%\} cause: \{\% else \%\} effect: \{\% endif \%\} & \multirow{4}{*}{\makecell[c]{\\3.00}} \\
% ~ & \textbf{BT}: - & ~ \\
% ~ & \textbf{GPT2}: - & ~ \\
% ~ & \textbf{T5}: Select the most agreeable \{\% if question == "cause" \%\} cause: \{\% else \%\} effect:\{\% endif \%\} & ~ \\
% \midrule
% \multirow{4}{*}{\makecell[c]{\\SuperGLUE \\ CB}} & \textbf{Origin}: \{\{premise\}\} Are we justified in saying that "\{\{hypothesis\}\}"? Yes, no, or maybe? & \multirow{4}{*}{\makecell[c]{\\5.36}} \\
% ~ & \textbf{BT}: - & ~ \\
% ~ & \textbf{GPT2}: - & ~ \\
% ~ & \textbf{T5}: \{\{premise\}\} If we were justified, would we think that it is the case that we are justified in saying that "\{\{hypothesis\}\}"? Yes, no, or maybe? & ~ \\


% \midrule
% \multirow{4}{*}{\makecell[c]{\\SuperGLUE \\ WSC}} & \textbf{Origin}: Passage: \{\{text\}\} Question: In the passage above, does the pronoun "\{\{span2\_text\}\}" refer to \{\{span1\_text\}\}? Answer: & \multirow{4}{*}{\makecell[c]{\\10.58}} \\
% ~ & \textbf{BT}: - & ~ \\
% ~ & \textbf{GPT2}: - & ~ \\
% ~ & \textbf{T5}: Passage: \{\{text\}\} Question: Is the pronoun "\{\{span2\_text\}\}" referring to the meaning of \{\{span1\_text\}\} ? Answer: & ~ \\


% \bottomrule
% \end{tabular}
% \caption{Illustration of prompts generated by GPS.}
% \label{tab:en-gps}
% \end{table*}


\begin{table*}[t]
\small
\centering
\begin{tabular}{m{1.4cm}<{\centering}p{12cm}m{1.0cm}<{\centering}}
\toprule
\textbf{Task} & \textbf{Generated Prompts} & \textbf{Metric} \\
\midrule
\multirow{4}{*}{\makecell[c]{\\ Hellaswag}} & \textbf{Origin}: If a description of a situation begins like this: \{\{ ctx \}\}... Then how does it continue? & 34.00 \\
~ & \textbf{BT}: If the description of a situation begins like this: \{\{ ctx \}\}... Then how will it continue? & 34.74 \\
~ & \textbf{SC(GPT2)}: - & 34.00 \\
~ & \textbf{SC(T5LM)}:  If a description of a situation begins like this: \{\{ ctx \}\}... then what is the most likely thing to happen next? & \textbf{47.63} \\
\midrule
\multirow{4}{*}{\makecell[c]{\\SuperGLUE \\ COPA}} & \textbf{Origin}: Select the most plausible \{\% if question == "cause" \%\} cause: \{\% else \%\} effect: \{\% endif \%\} & 93.00\\
~ & \textbf{BT}: Select the most believable \{\% if question == "cause" \%\} cause: \{\% else \%\} effect: \{\% endif \%\} & 95.00 \\
~ & \textbf{SC(GPT2)}: What is the most plausible \{\% if question == "cause" \%\} cause: \{\% else \%\} effect:\{\% endif \%\} & 95.00 \\
~ & \textbf{SC(T5LM)}: Select the most agreeable \{\% if question == "cause" \%\} cause: \{\% else \%\} effect:\{\% endif \%\} & \textbf{96.00} \\
\midrule
\multirow{4}{*}{\makecell[c]{\\SuperGLUE \\ CB}} & \textbf{Origin}: \{\{premise\}\} Are we justified in saying that "\{\{hypothesis\}\}"? Yes, no, or maybe? & 78.57 \\
~ & \textbf{BT}: \{\{premise\}\} Do we have reason to say this "\{\{hypothesis\}\}"? Yes, no, or maybe? & 83.93 \\
~ & \textbf{SC(GPT2)}: \{\{premise\}\} Are we justified in believing that "\{\{hypothesis\}\}"? Yes, no, or maybe? & 80.36 \\
~ & \textbf{SC(T5LM)}: \{\{premise\}\} If we were justified, would we think that it is the case that we are justified in saying that "\{\{hypothesis\}\}"? Yes, no, or maybe? & \textbf{83.93} \\


\midrule
\multirow{4}{*}{\makecell[c]{\\SuperGLUE \\ WSC}} & \textbf{Origin}: Passage: \{\{text\}\} Question: In the passage above, does the pronoun "\{\{span2\_text\}\}" refer to \{\{span1\_text\}\}? Answer: & 60.58 \\
~ & \textbf{BT}: Passage: \{\{ text \}\} Question: in the paragraph above, does the pronoun "\{\{ span2\_text \}\}" refer to \{\{ span1\_text \}\}? Answer: & 67.31 \\
~ & \textbf{SC(GPT2)}: - & 60.58 \\
~ & \textbf{SC(T5LM)}: Passage: \{\{ text \}\} Question: does the pronoun "\{\{ span2\_text \}\}" refer to the person of \{\{ span1\_text \}\}? Answer: & \textbf{70.19} \\


\bottomrule
\end{tabular}
\caption{Illustration of prompts generated by GPS. “-” indicates when the score of the original prompt is better than the generated prompts, and GPS will keep the original prompt as the final result.}
\label{tab:en-gps}
\end{table*}



\subsubsection{The Size of Validation Set}

% \begin{table}[t]
% \small
% \centering
% \begin{tabular}{cccccc}
% \toprule
% Val Size & 8 & 16 & 32 & 64 & 128\\
% % \midrule
% % ANLI R1    & 43.56 & 42.60 & 43.04 & 49.56 & 37.58 & & 46.47\\
% % ANLI R2    & 38.68 & 38.94 & 38.19 & 42.53 & 33.05 & & 39.91\\
% % ANLI R3    & 41.26 & 41.34 & 40.48 & 42.59 & 38.98 & & 43.01\\
% % CB         & 70.12 & 71.90 & 74.05 & 77.98 & 65.24 & & 80.00\\
% % RTE        & 80.83 & 82.01 & 82.92 & 81.30 & 72.42 & & 83.86\\
% % WSC        & 61.45 & 60.38 & 63.56 & 65.87 & 64.42 & & 65.48\\
% % Winogrande & 59.94 & 59.24 & 58.00 & 58.92 & 51.45 & & 61.96\\
% % COPA       & 90.02 & 91.13 & 93.02 & 93.17 & 84.07 & & 93.43\\
% % HellaSwag  & 33.55 & 33.38 & 46.90 & 47.23 & 32.25 & & 51.83\\
% % WiC        & 56.68 & 57.37 & 57.98 & 59.14 & 49.33 & & 58.82\\
% \midrule
% Avg        & 60.57 & 61.35 & 62.48 & 62.40 & -\\
% \bottomrule
% \end{tabular}
% \caption{Ablation results on the size of validation set.}
% \label{tab:ablation_val_size}
% \end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/GPS_ablation_val_size.pdf}
    \caption{Ablation results on the size of the validation set. The performance with an empty validation set is zero-shot T0.
}
    \label{fig:ablation_val_size}
\end{figure}

The validation set plays an important role in GPS for scoring each prompt, and its size matters to give credible feedback for the prompt selection. 
The results of GPS on validation sets of different sizes from 8 to 128 are presented in Fig.~\ref{fig:ablation_val_size}. Generally, the gain of prompt search rises with more validation samples. Most datasets follow this trend, such as WSC and HellaSwag. Although more examples lead to further improvement, we set the default size of validation set to 32 in our experiments because we focus on the few-shot scenario with limited labeled points. The size of the prompt pool might be important as well for continuous improvement, especially with a large validation set. Here we set the prompt pool size to be 30 in consideration of the computational costs. On the other hand, GPS is still much better than manual prompts when there is only 8 examples for validation.


\subsubsection{The Number of Prompt Search Iterations}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/GPS_ablation_num_iter.pdf}
    \caption{Ablation results on the number of prompt search iterations. The performance with 0 iterations is zero-shot T0.
}
    \label{fig:ablation_num_iter}
\end{figure}

Another critical hyperparameter is the number of iterations for genetic prompt search. We experimented with up to 9 prompt sesarch iterations and the results are given in Fig.~\ref{fig:ablation_num_iter}. It can be seen that the performances on some datasets such as WSC and Winogrande achieve the best at an early iteration. However, the overall performance on all the datasets improves on more search iterations. The default iteration number is set to 6 in the paper for the trade-off between the performance and costs. 

\begin{table*}[t]
\small
\centering
\begin{tabular}{cm{0.8in}<{\centering}m{0.8in}<{\centering}m{0.8in}<{\centering}m{0.8in}<{\centering}}
\toprule
% \multirow{2}{*}{Methods} & \multirow{2}{*}{Serving \\Efficiency} & \multirow{2}{*}{Tunable \\Parameters} & \multirow{2}{*}{Performance} & \multirow{2}{*}{Computation cost \\FLOPs}\\
Methods & Serving Efficiency & Tunable Parameters & Performance & Computation Cost$^\dag$\\
\midrule
Model Tuning         & \xmark & 100\%         & 61.73 & 11.1x \\
Prompt Tuning        & \cmark & $\sim$ 0.01\% & 58.56 & 11.1x \\
Black-Box Tuning     & \cmark & $\sim$ 0.001\%  & 57.82 & 9.3x \\
In-Context Learning  & \xmark$^\ddag$ & 0\%           & 51.28 & 0x \\
our GPS              & \cmark & 0\%           & 60.12 & 1.0x \\
\bottomrule
\end{tabular}
\caption{Overall comparison of different few-shot learning methods on serving efficiency, tunable parameters, performance and computation cost. $\dag$: Computation cost here refers to the combined cost of training and prompt search. $\ddag$: In-context learning uses a long sequence length to concatenate examples, which is expensive for inference.}
\label{tab:overall_comparison}
\end{table*}

% \subsubsection{Size of the Prompt Pool}

% TODO:table 2 和tabel3顺序应该交换一下，因为case study章节在后面
\subsection{Case Study} 
\label{sub:case_study}
In Table \ref{tab:en-gps}, we present cases of prompts selected by GPS using different strategies. As we can see, GPS modifies the original prompts to optimize performance for unseen tasks while not changing the major meanings.
% of the sentences.
However, using simple strategies like back translation can only provide minor prompt modifications, while SC with T5LM shows larger prompt modifications and dramatically better performance. 
For example, in WSC, GPS firstly removes the less informative adverb ``In the passage above'', and then adds a hint ``the person of'' to help the model navigate the answer. This modification obtains a significant 10 points gain compared to the original prompt. 
Overall, Table~\ref{tab:en-gps} illustrates the necessity and effectiveness of \proposed, especially when SC is used on a large language model.

\subsection{Overall Comparison of Different Few-Shot Methods}


Table~\ref{tab:overall_comparison} compares different methods on serving efficiency, tunable parameters, performance, and computational cost.
% Note that all methods except for In-Context Learning use the same number of labeled data points. In-Context Learning takes only 2-shot due to the limited GPU memory.

\textbf{Serving Efficiency.} MT lacks serving efficiency due to the huge storage cost to store the full model for each new task. Although ICL does not have any tunable parameter, the long sequence length makes it expensive for inference, especially when the number of demonstrations is large. PT, BBT and GPS have few or zero tunable parameters, and thus they are cheaper for deployment.
% Note that it might be expensive to use soft-prompt based methods when the length of soft prompt is large, especially for short text classification tasks.

\textbf{Tunable Parameters.} MT needs to tune the full model for each task, and it requires large resources because the commonly-used optimizers such as Adam require to store extra momentum and variance terms. PT and BBT only tune the prompt embeddings and are more efficient.
ICL and GPS are the most parameter-efficient as they require no parameter updating.

\textbf{Performance.} GPS has the second best performance even though all the model parameters are frozen. MT is better than PT, and PT is better than BBT, which is different from the results given in~\citet{Sun2021blackbox}. We suppose the reason is that we use different pretrained models and test datasets, and a more strict setting where only 16 examples are used for the train and dev set, respectively.

\textbf{Computational Cost.} We consider the computational cost as the number of equivalent forward passes during the training or the prompt search stage. 
The training batch size for MT and PT is 4 and the total training step is 4000. 
We estimate the computational cost for each backward pass as two forward passes. 
The number of the manual prompts and the topK for prompt selection are both 5.
For BBT, the training iteration is 500 and the prompt number is 5, and we omit the cost of CMA-ES. For GPS, we consider 6 search iterations and a prompt pool size of 30, the cost for generating one prompt is estimated as two forward passes.
In total, the equivalent computation costs for MT and PT are 48000 forward passes, and they are 40000 and 4320 for BBT and GPS, respectively.

Overall, our GPS has good serving-efficiency, low computation cost, does not have any tunable parameter, and still achieves the best performance. It can be a promising option for a large-scale NLP production system to improve the performance of pretrained language models with only limited labeled examples.


\section{Conclusions}
In this paper, we propose \proposed, an automatic prompt search method based on genetic algorithm for better few-shot learning. We compare different approaches on 10 datasets with only 32 labeled examples available. \proposed outperforms not only the manual prompt baseline, but also other parameter-efficient few-shot learning methods. Extensive experiments verified the effectiveness of the proposed \proposed.


\section{Limitations}

We show that Genetic Prompt Search is an efficient few-shot learning approach with competitive performance as well as low cost.
Our results have a few limitations, however, and it is possible that few-shot performance could be further improved by studying those problems in the future.
Specifically, 
1) We conduct experiments on the T0 benchmark with 10 test datasets. It is not clear how our method performs on other datasets.
% and our results are not generally applicable for all NLP problems. The effectiveness of GPS for diverse downstream tasks still needs exploring.
2) We only compare different methods under the few-shot setting with 32 examples in total. Conclusions regarding the performance of different methods might be different with more labeled examples. For example, if it is possible to get hundreds of or even thousands of training examples, tuning-based methods might achieve much better and more stable performance.
3) Although GPS is able to find better prompts automatically, it is still not clear why these prompts work better. Further research on the mechanism of prompting on large-scale language models can help us understand what kind of prompt works and how to design optimal prompts.
We hope our results could encourage future work on addressing these limitations to further explore the potential of few-shot learning.





% Entries for the entire Anthology, followed by custom entries
\bibliography{custom}
\bibliographystyle{acl_natbib}


==> EMNLP 2022/intro.tex <==
\section{Introduction}


Pretrained language models, such as BERT \cite{devlin-etal-2019-bert}, XLNet \cite{yang2019xlnet}, T5 \cite{JMLR:v21:20-074}, and GPT \cite{radf2019lmmultitask}, are often finetuned for downstream natural language processing tasks, which has been shown to improve performance over non-pretrained models. However, this pretraining-finetuning paradigm still relies on a relatively large set of labeled data for each downstream task to obtain competitive performance. 
Although GPT-3 \cite{NEURIPS2020_gpt3} shows promising performance for zero-shot and few-shot learning by prompting on an extremely-large pretrained language models with 175B parameters,
% done: 连续两个however开头的句子
finding out the optimum prompt for each given task could be difficult~\cite{mishra2021reframing,wang2022language}.

To improve the performance of prompting on pretrained language models, recent works focus on supervised pretraining with carefully designed or crowdsourced manual prompts~\cite{eval-harness,wei2021finetuned,sanh2021multitask,Ouyang2022InstructGPT}.
% To achieve the best performance, ~\citet{wei2021finetuned} made efforts on careful prompt design.
Diverse prompts are collected to enhance the robustness and performance of prompting~\cite{sanh2021multitask}. \citet{Ouyang2022InstructGPT} introduced a dataset of labeler demonstrations and used it to finetune GPT-3.
Despite all these efforts, the challenge to obtain high-performing prompts for few-shot learning still exists. 
As pointed out by previous works \cite{liu2021gpt,gao-etal-2021-making,liu2021pre}, manual prompts are usually suboptimal and suffers a high variance on performance.
% done: also这里是不是应该断句
% On the other hand, tuning-based methods including finetuning the full model or tuning only part of the parameters~\cite{lester2021power} calls for high computation costs. Full model tuning is also difficult to serve due to its large storage cost of model parameters.


\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{EMNLP 2022/figures/prompts_GPS_v2_re.pdf}
    \caption{The paradigms of Model Tuning, Prompt Tuning, and \proposed. Model Tuning requires the pretrained model to be tunable, and the tuned model can be only used for a single task. Prompt tuning needs extra tunable soft prompts. Our proposed \proposed is tuning-free.}
    \label{fig:intro_GPS}
\end{figure*}

To address this challenge, we propose a novel Genetic Prompt Search (\proposed) algorithm that gradually mutates the prompts with a generative model and selects candidates according to their performance on a small development set. This evolutionary procedure relies on a tiny set of labeled data, only used for validation but not training.
% GPS enjoys the benefit of automatically finding high-performing prompts with only a few validation samples. 
As illustrated in Figure~\ref{fig:intro_GPS}, GPS does not require updating any parameter, but only searches for the optimal hard prompts for every downstream task.
% while model tuning requires a huge amount of computation resources for updating model parameters and is only capable of serving to one specific task after the tuning process. 
% Also, prompt tuning calls for extra soft prompts as input, and the parameters of the soft prompts are updated during the training process. 
% Whereas, GPS does not require any parameter update and the genetic search of prompts can be regarded as a combination of both tunable soft prompt and hard manually designed prompts. 
% while Comparing to previous methods like P-tuning~\cite{liu2021gpt}, model tuning or priming~\cite{NEURIPS2020_gpt3}, GPS obtain better performance with fewer computational cost. 
Similar to prompt tuning, \proposed allows the pretrained model to serve a large number of applications simultaneously. Meanwhile, \proposed is even easier to deploy than prompt tuning, because it does not need to store the tuned continuous soft prompts. 
% since it does not need to update parameters of the base model. 
% GPS not only improves the performance compared to manual prompts under the ``zero-shot adaptation with few-shot validation'' setting. 
% Furthermore, GPS can be integrated with other model tuning and prompt tuning approaches of further performance boost under the few-shot learning setting. 
% In addition to the genetic prompt search, \proposed also explores several other possibilities such as prompt design for multitask learning. 
% TODO: 感觉效果这块应该强调一个是比manual prompt提升巨大，另外*甚至*要比model tuning还高
Empirically, \proposed achieves substantial improvement over the baseline of manual prompts, and it also outperforms other parameter-efficient few-shot tuning methods.
% We also study the effect of different prompt generation strategies including back translation and cloze, sentence continuation by using pretrained language models.
% both strong zero-shot learning and supervised tuning baselines. 

% done: contributions一般写3点比较好。1. 我们提出了gps，可以在不训练的情况下提升效果
% 2. 我们实验证明了手工的prompt通常很差，即使用一些简单的方法比如back translation也能显著提升手写prompt的效果。而我们的方法比manual提升显著。同时我们还对比了其他fewshot的方法。我们的方法不仅轻量而且效果甚至能比mt还要好
% 3. 我们通过细致的分析实验证明了我们方法的计算效率以及超参数的影响，同时case分析证明了我们搜出来的参数不仅效果还还是语意流畅的。（相比于auto prompt之类的方法搜出来的结果没有实际语义）
Our contributions can be summarized as follows. 
\begin{itemize}
    % with an extremely large number of tasks, model size has little impact on performance.
    \item We propose a tuning-free Genetic Prompt Search method that only requires a small validation set to automatically search for high-performing prompts.
    \item Our experiments demonstrate that manual prompts are usually suboptimal. Using the proposed search method, some simple augmentation technique such as back translation can lead to considerable improvement over manual prompts. Further, our best practice outperforms parameter-efficient few-shot tuning baselines. We conduct an overall comparison of different few-shot learning methods, and our proposed method stands out with the best performance as well as serving efficiency.
    \item We carefully studied the effects of hyper-parameters and prompt generation strategies in the proposed algorithm. Different from previous work~\cite{shin-etal-2020-autoprompt}, we find that our searched prompts are semantically fluent just as human-written templates.
\end{itemize}

==> EMNLP 2022/method.tex <==
\section{Genetic Prompt Search}
% We follow the same framework of multitask zero-shot learning in ~\cite{wei2021finetuned,sanh2021multitask}, where models are pretrained on a variety of tasks and then tested on held-out unseen tasks. 
% TODO: 这里表述有点问题，我们只有一个setting，就是32 validation，应该算是fewshot
% The Genetic Prompt Search is proposed for both zero-shot and few-shot learning setting. For the zero-shot setting, a tiny validation set is occupied for automatically find the optimum prompt. While for the few-shot setting, the dataset will be split to train and validation set with equal number of samples. 

% Comparing to previous zero-shot or few-shot learning approaches~\cite{liu2021gpt,wei2021finetuned,sanh2021multitask}, updating the parameters in the production setup relies on much more challenging engineering efforts compared to using a frozen model, especially when the model is large. 
% Moreover, as we will show in the experiments, few-shot prompt tuning is much more computationally expensive than our approach.


In this section, we will introduce the algorithm of Genetic Prompt Search (GPS) and various prompt generation strategies we have studied. Note that the prompt search here refers to the search for a high-performing hard prompt in the discrete word space as shown in Fig.~\ref{fig:intro_GPS}, and the formulation does not include soft prompts.


% \subsection{Manual Prompts}

% The \proposed method calls for the pretrained language model in both search and inference phase. Empirically, we can choose strong baselines that fit for the zero-shot learning scenarios, like T0~\cite{sanh2021multitask} or GPT-3~\cite{NEURIPS2020_gpt3}. 

% % In this paper, \proposed under the multitask learning setting, since \proposed can be used directly for all kinds of training tasks. 
% As mentioned in Figure~\ref{fig:gps_main}, the \proposed calls for some handcrafted prompts in the beginning as initialization. In our experiment, our initial prompts are collected from the T0 project where prompts are manually created in the crowd-sourcing manner. Also, since \proposed can be used directly for all kinds of training tasks, we will experiment \proposed in different kinds of tasks types like NLI and sentence completion. 
% . As mentioned in~\cite{wang2022language}, crowd-sourcing prompts are often sub-optimal, and we believe \proposed can 


% In T0, prompts are used in the multitask finetuning phase, . However, we choose these crowd-sourced prompts as the seed prompts and will search for the best prompts using \proposed. 
% To be more specific, \proposed will start adapt 

\subsection{Genetic Prompt Search Algorithm}
\label{subsection:genetic_prompt_search}
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.75\textwidth]{figures/prompt_design.pdf}
%     \caption{The hybrid prompt composed of task-specific soft prompt, verbalizer prompt and task description prompt.}
%     \label{fig:prompt_design}
% \end{figure*}



% Previous works on automatic prompt generation are well-studied in the few-shot learning settings~\cite{shin-etal-2020-autoprompt,gao-etal-2021-making}, whereas in our paper we focus on few-shot validation.
% For a new task, we want to automatically obtain high-performing prompts without updating model parameters.
% Inspired by Genetic Algorithms~\cite{mitchell80}, we propose Genetic Prompt Search (GPS) to further improve the performance of \proposed.
It is challenging to automatically find high-performing prompts for a new unseen task.
Inspired by Genetic Algorithms~\cite{mitchell80}, we propose Genetic Prompt Search (GPS) for this purpose.
% to automatically obtain high-performing prompts.

% Following a more realistic zero-shot learning setting~\cite{keung2020don}, 
In \proposed, we will first sample a tiny number of data as a development set $D_{dev}$ for each downstream task. 
% We term this setting as ``zero-shot adaptation with few-shot validation".
Then, we will design two genetic functions, where $f_{GPS}$ is the metric function to decide which prompts will be reserved or eliminated at each iteration, and $g_{GPS}$ represents the genetic function to generate new prompts.
% TODO: 这里figure，不是Algorithm
% TODO: 我们用的是全部的manual prompt，不是3个
The process of Genetic Prompt Search is described in Fig.~\ref{fig:gps_main}.
According to the algorithm, GPS is firstly initialized with a set of handcrafted prompts, $G^0$.
% In practice, we can achieve good performance with 3 prompts for initialization. 
And the key process of GPS is to reproduce the current generation of prompts and use re-scoring to select prompts iteratively. 
For each iteration, we calculate the scores of prompts in $G^t$ using $f_{GPS}$, and select the top-$K$ prompts as $G^t_*$. 
Then we generate $G^{t+1}$ using $g_{GPS}$ based on $G^t_*$.
After several steps of genetic search, we will collect all the top-$K$ prompts in each generation, and rescore all these prompts to make the final decision on which prompts are optimal.

Now we discuss several strategies to generate the candidates at each iteration.


%   choose one organization that requirr
% Algorithm~\ref{alg:ga-Framwork}
% The algorithm is firstly initialized with a set of handcrafted prompts $G^0$. In practice, we can achieve good performance with 3 prompts for initialization. 
% For each iteration, we calculate the scores of prompts in $G^t$ using $f_{GPS}$, and select the top-$K$ prompts as $G^t_*$. 
% Then we generate $G^{t+1}$ using $g_{GPS}$ based on $G^t_*$.
% Finally, we select the top-$K$ prompts from all prompts.

% \subsection{GPS with Updating Parameters}
% Except dealing with the ``zero-shot adaptation with few shot validation'' problem, GPS can also be combined with normal prompting approaches for few-shot learning, where part or all of the parameters can be updated. 
% % in natural language processing settings, where parameters can be updated. 

% As mentioned before, GPS can easily be adapted to prompt and model tuning, as well as priming. 
% For both model and prompt tuning method, we divide the prompts to two parts, hard and soft prompts. Where the hard prompts are manually written by experts, and the soft prompts are randomly initialized embeddings. 
% For the hard prompts, we use the GPS algorithm to find the optimum hard prompt.
% While we use prompt tuning or model tuning to optimize the soft prompt. 

% We will first tune the model with soft prompts and use the tiny validation set to search for the optimum 
% When using the GPS, 
% For prompt tuning, we use the GPS first, and prompt tuning 

% For model tuning, GPS is used similar to prompt tuning. 

% For the priming work, we firstly design our basic prompts, and concat the examples into the prompts. In the searching stage, we only search the prompts token, while the examples will not change. 



\subsection{Prompt Generation Strategies}
\label{subsection:prompt_generation}

\begin{algorithm}[t]
  \caption{Genetic Prompt Search}  
  \label{alg:ga-Framwork}  
  \begin{algorithmic}[1]
    \Require  
      $G^0$; $D_{dev}$; $f_{GPS}$; $g_{GPS}$; $T$; $K$;
    \Ensure  
      Final optimized prompts, $G^{T+1}$
    \State obtain handcrafted prompts $G^0$ as initialization
    \For{each $t\in [0,T]$}
        \State store $G^t$
        \State calculate score for each prompt in $G^t$ using $f_{GPS}$,
        \State from $G^t$, select top $K$ prompts as reproductive group $G^t_*$,
        \State generate $G^{t+1}$ based on $G^t_*$ using $g_{GPS}$,
    \EndFor
    \State from stored $\{G^0_*,...,G^T_*\}$, select top $K$ prompts as optimal prompts group $G^{T+1}$ using $g_{GPS}$ . \\
    \Return $G^{T+1}$;  
  \end{algorithmic}  
\end{algorithm}

\textbf{Back Translation}: Back Translation (BT), a common technique for data augmentation in NLP, is applied for prompt reproduction. Here we first translate the manual prompts from English to 11 other languages including Chinese, Japanese, Korean, French, Spanish, Italian, Russian, German, Arabic, Greek, Cantonese, and then translate them back to English.

\textbf{Cloze}: We introduce a prompt generation approach making use of the cloze task form and pretrained language models. Firstly, we follow previous work LM-BFF~\cite{gao-etal-2021-making}, which is a suite of simple techniques for few-shot learning, and exploit its automatic template generation method. Specifically, we use the large pretrained text-to-text transformer (T5)~\cite{JMLR:v21:20-074} to generate templates. For each input example and its verbalizer, we compose the template with placeholders as prefix and suffix, and let T5 to fill in the placeholders. We apply beam search to generate multiple prompt candidates. More details can be found in~\citet{gao-etal-2021-making}. However, this approach does not work well since our setting conducts no parameter update, which is different from the few-shot training setting in the original paper. Therefore, we instead use manual prompts as initial templates, replace some random tokens with placeholders, and then let T5 fill in the blanks to generate new prompts. We select the best prompt according to the average logits across all the validation samples.

\textbf{Sentence Continuation}: Another alternative for prompt augmentation is Sentence Continuation (SC). Inspired by DINO~\cite{schick2020generating},
% where the pretrained language model is used to generate data samples,
we use a pretrained language model to generate new prompts. Specifically, we use the template ``Write two sentences that mean the same thing. Sentence 1: \textit{Manual Prompt}, Sentence 2:" to the pretrained model, and let it generate continuations as a new prompt. We conducted experiments with GPT2-XL (1.5B) and T5LM-XXL (11B) as our prompt generation models.

\textbf{Prompt Scoring}:
For Cloze, we follow previous work~\cite{gao-etal-2021-making} to score the prompts with average logits on the validation set $D_{dev}$. For Back Translation and Sentence Continuation, since averaging logits is not applicable, we score each prompt using accuracy on $D_{dev}$.

==> EMNLP 2022/related.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.99\textwidth]{EMNLP 2022/figures/GPS_main.pdf}
    \caption{Overall pipeline of our GPS algorithm. The idea of GPS is borrowed from the genetic algorithm. Prompts are initialized from handcrafted prompts. Better prompts are searched for over each iteration. Finally, all generated prompts are reranked and selected as the final prompts. }
    \label{fig:gps_main}
\end{figure*}

%  Overall Pipeline of GRIPS. The main steps are numbered. Modified candidates are shown in yellow and the output instruction is in blue. We use ‘[ ]’ to show the syntactic phrase-level splits at which the edit operations occur. Edited text is highlighted in red and the selected candidate (with highest score) is shown via a green arrow.
\section{Related Work}
Recently, thanks to the prompt-based learning method, pretrained language models (PLMs) have been widely explored under zero-shot and few-shot scenarios for language understanding and generation tasks~\cite{schick-schutze-2021-exploiting,gao-etal-2021-making,le-scao-rush-2021-many}.
% TODO: augmenting意思确认对吗？
Prompt-based learning bridges the gap between pretraining and finetuning objectives by stitching the text input $X$ with a prompt template and augmenting the label output $y$ as a text string, such that the input and the output can be constructed in a sentence completion task form.
Previous few-shot learning methods can be generally categorized into two types, few-shot tuning methods that require updating parameters~\cite{liu2021gpt,han2021ptr} and prompt enchancement methods that have no learnable parameter but optimize the discrete prompts directly~\cite{shin-etal-2020-autoprompt,mishra2021reframing}.

\subsection{Few-Shot Tuning}
Some few-shot tuning methods focus on template design and update all the parameters of pretrained language models. PET\cite{schick-schutze-2021-exploiting} exploited the simple manual template and unified different classification tasks with pattern-verbalizer pairs. LM-BFF~\cite{gao-etal-2021-making} proposed several simple techniques for better few-shot learning including automatic verbalizer search and automatic prompt search. \citet{han2021ptr} applied rules in prompt tuning to deal with the hard many-class text classification tasks.

Another line of work is parameter-efficient few-shot learning, which aims at reducing the number of tunable parameters to improve deployment efficiency. Adapters~\cite{pmlr-v97-houlsby19a} proposed to add an adpater module integrated in the original language model for each downstream task and only this module is tunable. \citet{lester2021power} showed the effectiveness of tuning the prompt embeddings only especially for large-scale models.
P-tuning~\cite{liu2021gpt} applied continuous prompt embedding optimization for GPT and made it comparable to BERT on NLU tasks.
BitFit~\cite{ben-zaken-etal-2022-bitfit} tuned only the bias terms of the original model. A low-rank decomposition approach named LoRA was proposed in \citet{Hu2021LoRA}, which injected trainable matrices in parallel with the original forward pass into each layer.
Black-Box Tuning~\cite{Sun2021blackbox} is a gradient-free optimization method for prompt tuning and thus it is suitable to use language models as a service.
%done: on the other hand应该用于并列关系，一般后面跟的不是转折关系
However, all these aforementioned methods require updating parameters, which is computationally expensive and costly in storage capacity for serving every task at hand. Our \proposed, instead, is tuning-free and aims at searching for the optimal prompts. 


\subsection{Prompting Enhancement}
GPT-3~\cite{NEURIPS2020_gpt3} shows the effectiveness of In-Context Learning. However, discrete prompting requires human efforts to provide manual prompts, and its sensitivity to labeled examples makes it hard to obtain stable performance.
AutoPrompt~\cite{shin-etal-2020-autoprompt} proposed to search discrete prompts with a gradient-guide method, but the generated prompts are literally uninterpretable. GPTk~\cite{mishra2021reframing} explored several ways to manually reframe task instructions.
% TODO: grips的讨论应该多一点。
% 在本文完成之前，有同时期的工作被放出来--grips。该方法同样使用了演化算法类似的思想。该算法每次使用增删改查来修改prompt。与grips方法相比，我们的方法使用lm来生成语义相似的prompt，不仅避免了手工定义修改规则，并且生成出来的prompt是语义流畅的。我们在实验中浮现了grips并进行了实验效果的对比.

GRIPS~\cite{prasad2022grips} is a concurrent work, which also applies iterative prompt search to improve the few-shot performance. Several operations, including add, deletion, swap and paraphrase, are defined to edit the manual prompts. Compared to GRIPS, our method uses different prompt reproduction approaches including back translation as well as cloze and sentence continuation by using generative language models. These methods do not need any human-defined edit rule and the generated prompts are semantically fluent. We conduct experiments comparing the performance of GRIPS and our method in Sec~\ref{sec:exp}.

In this paper, we follow T0~\cite{sanh2021multitask}, which is a very powerful zero-shot baseline of multitask prompted training.
Different from T0 and other methods, we regard the crowd-sourced manual prompts as seed prompts, and focus on parameter-free and gradient-free prompt search to further improve prompting performance under the few-shot learning setting.


